GauS-SLAM: Dense RGB-D SLAM with Gaussian Surfels

We propose GauS-SLAM, a dense RGB-D SLAM system that leverages 2D Gaussian surfels to achieve robust tracking and high-fidelity mapping. Our investigations reveal that Gaussian-based scene representations exhibit geometry distortion under novel viewpoints, which significantly degrades the accuracy of Gaussian-based tracking methods. These geometry inconsistencies arise primarily from the depth modeling of Gaussian primitives and the mutual interference between surfaces during the depth blending. To address these, we propose a 2D Gaussian-based incremental reconstruction strategy coupled with a Surface-aware Depth Rendering mechanism, which significantly enhances geometry accuracy and multi-view consistency. Additionally, the proposed local map design dynamically isolates visible surfaces during tracking, mitigating misalignment caused by occluded regions in global maps while maintaining computational efficiency with increasing Gaussian density. Extensive experiments across multiple datasets demonstrate that GauS-SLAM outperforms comparable methods, delivering superior tracking precision and rendering fidelity. The project page will be made available at https://gaus-slam.github.io.

==> sec/table/TUM_tracking_performance.tex <==
\begin{table}
\centering
 
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \texttt{fr1/desk} & \texttt{fr2/xyz} & \texttt{fr3/office} & \textbf{Avg.} \\
\midrule
\rowcolor{gray} \multicolumn{5}{l}{NeRF-based} \\
Nice-SLAM\cite{Nice-SLAM} & 4.26 & 6.19 & 3.87 & \\
Point-SLAM\cite{Point-SLAM} & 4.34 & 1.31 & 3.48 & \\
\rowcolor{gray} \multicolumn{5}{l}{Gaussian-based (decoupled)} \\

\rowcolor{gray} \multicolumn{5}{l}{Gaussian-based (coupled)} \\

\bottomrule
\end{tabular}
}
\caption{\textbf{Performance on TUM-RGBD.}}
\label{table:TUM_performance}
\end{table}

% Our approach achieves comparable performance on the TUM-RGBD\cite{TUM-RGBD} and ScanNet\cite{ScanNet} datasets, and outperforms existing methods on the ScanNet++\cite{scannetpp} dataset. 

==> sec/table/ablation_study_on_keyframe_localmap.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\textbf{KeyFrame} & \textbf{LocalMap} & \textbf{ATE} & \textbf{PSNR} & \textbf{Avg.Freq} \\
\textbf{Thresh} & \textbf{Thresh} & [cm]$\downarrow$ & [dB]$\downarrow$ & [Hz]$\uparrow$ \\
\midrule
\textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & 2.95 & 2.15 & 25.40 \\
0.01 & 1.5 & 1.30 & 0.74 & 31.36 \\
0.05 & 1.5 & \textbf{0.27} & \textbf{0.49} & \textbf{32.81} \\
0.10 & 1.5 & \textbf{0.27} & \textbf{0.49} & \textbf{32.81} \\
0.05 & 2.0 & \textbf{0.27} & \textbf{0.49} & \textbf{32.81} \\
0.05 & 3.0 & \textbf{0.27} & \textbf{0.49} & \textbf{32.81} \\
\bottomrule
\end{tabular}
}
\caption{Experimental Results Table}
\label{tab:results}
\end{table}

==> sec/table/reconstruction_performance.tex <==

\begin{table}[h!]
\centering
\caption{Rendering Performance on Replica. We outperform all existing dense neural RGBD methods on the commonly reported rendering metrics. The numbers for NICE-SLAM and Vox-Fusion  are taken from.}
\begin{tabularx}{0.48\textwidth}{p{0.8cm}p{1.2cm}*{9}{>{\raggedright\arraybackslash}X}}
\toprule
\textbf{Method} & \textbf{Metric} & \textbf{R0} & \textbf{R1} & \textbf{R2} & \textbf{O0} & \textbf{O1} & \textbf{O2} & \textbf{O3} & \textbf{O4} & \textbf{Avg.} \\ \midrule
\multirow{2}{*}{ESLAM} 
& Depth L1 [cm]$\downarrow$ & 0.63 & 0.62 & 0.98 & 0.57 & 1.66 & 7.32 & 3.94 & 0.88 & 2.08\\
& F1 [\%]$\uparrow$    & 80.3 & 81.1 & 83.7 & 79.4 & 73.9 & 75.9 & 75.6 & 76.2 & 78.2\\ 
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{2}{*}{\makecell[l]{Point-\\SLAM\cite{Point-SLAM}}} 
& Depth L1 [cm] $\downarrow$ & 0.53 & 0.22 & 0.46 & 0.30 & 0.57 & 0.49 & 0.51 & 0.46 & 0.44\\
& F1 [\%] $\uparrow$    & 86.9 & 92.3 & 90.7 & 93.7 & 91.6 & 88.9 & 88.2 & 85.5 & 89.7\\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{2}{*}{\makecell[l]{GS-\\SLAM\cite{GS-SLAM}}} 
& Depth L1 [cm] $\downarrow$ & 1.31 & 0.82 & 1.26 & 0.81 & 0.96 & 1.41 & 1.53 & 1.08 & 1.16\\
& F1 [\%]      $\uparrow$    & 62.8 & 79.8 & 66.8 & 80.0 & 81.5 & 65.9 & 59.1 & 64.9 & 70.1\\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{2}{*}{\makecell[l]{Gaussian-\\SLAM\cite{Gaussian-SLAM}}} 
& Depth L1 [cm] $\downarrow$ & 0.69 & 0.33 & 0.83 & 0.52 & 0.46 & 5.43 & 3.74 & 0.47 & 1.56\\
& F1 [\%]      $\uparrow$    & 88.0 & 90.2 & 88.9 & 92.0 & 90.5 & 83.9 & 81.4 & 86.2 & 87.6\\ 
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{2}{*}{\makecell[l]{GLC-\\SLAM\cite{GLC-SLAM}}} 
& Depth L1 [cm] $\downarrow$ & 0.57 & 0.24 & 0.50 & 0.44 & 0.48 & 1.06 & 1.85 & 0.45 & 0.70\\
& F1 [\%]      $\uparrow$    & 89.3 & 91.3 & 90.5 & 92.3 & 90.0 & 87.7 & 84.4 & 87.3 & 89.1\\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{2}{*}{\makecell[l]{\textbf{Ours}}} 
& Depth L1 [cm] $\downarrow$ & 1.31 & 0.82 & 1.26 & 0.81 & 0.96 & 1.41 & 1.53 & 1.08 & 1.16\\
& F1 [\%]      $\uparrow$    & 91.3 & 91.9 & 90.6 & 93.5 & 89.9 & 88.7 & 59.1 & 64.9 & 70.1\\
\bottomrule
\end{tabularx}
\end{table}
